NN-PARS: A Parallelized Neural Network Based Circuit Simulation Framework

The shrinking of transistor geometries as well as the increasing complexity of integrated circuits, significantly aggravate nonlinear design behavior. This demands accurate and fast circuit simulation to meet the design quality and time-to-market constraints. The existing circuit simulators which utilize lookup tables and/or closed-form expressions are either slow or inaccurate in analyzing the nonlinear behavior of designs with billions of transistors. To address these shortcomings, we present NN-PARS, a neural network (NN) based and parallelized circuit simulation framework with optimized event-driven scheduling of simulation tasks to maximize concurrency, according to the underlying GPU parallel processing capabilities. NN-PARS replaces the required memory queries in traditional techniques with parallelized NN-based computation tasks. Experimental results show that compared to a state-of-the-art current-based simulation method, NN-PARS reduces the simulation time by over two orders of magnitude in large circuits. NN-PARS also provides high accuracy levels in signal waveform calculations, with less than $2\%$ error compared to HSPICE.

==> variation.tex <==

\section{Process Variation PLEASE DON'T READ} \label{sec:process-variation}

As technology geometries continue to shrink to nano-meter scale, the ability to control critical device parameters is becoming increasingly difficult. This includes the dimensions, doping concentrations, orientation of metal grains and etc. Beside continuous technological improvements in creating new devices with more advanced fabrication processes, the problem of timing analysis under process variation is becoming more challenging and more accurate modeling is inevitable to accomplish timing and yield requirements. 

There are two main categories of process variations: (1) Systematic variation are deterministic in nature and can be attributed to the layout or fabrication equipment related effects. Thus they generally show spatial correlation behaviour in the chip (2) Random or non-systematic variation are unpredictable in nature, such as dimensions of gate/Fin (length, width, oxide thickness), doping fluctuation and even orientation of fabrication particles. Variations of this sort can vary independently for each device on a chip. 

There are other ways of classifying process variation such as intra or inter die, and front or back end variations, which are not the focus of this article. % Do I really need this? 

Manufacturer provides the information of process variation alongside the technology files. The number of parameters with process variation are vast. While most of these parameters are representing real physical features, some are fitting variables and don't have any physical meaning. To make sure the circuit work in different situations, Monte Carlo simulation is done. 

Considering the large number of parameters, the time complexity of Monte Carlo simulation is too much. This is why the status quo is to limit the process variation parameters to the most important ones to be able to do simple (maybe pre-final) simulations. The impact and type of sources are variation are different between technologies. As an example of new fabrication technology, by spacer lithography becoming prevalent for the last few years, the impact of Line Edge Roughness (LER) is not significant source of variation in FinFET devices. Moreover, while random dopant fluctuation (RDF) is a dominant in bulk planar MOSFET devices, it's impact does not exist in undoped FinFET devices. Replacing polysilicon with metal-gate resolved the various difficulties of using high-K materials and increased the $I_{ON}$ current of the devices. However, the metal work function is very dependent on the orientation of metal grains which is not controllable during the growth period and is then random. With the scaling of the gate area, it is expected to have about (\textasciitilde 10 \textasciitilde 100) of grains and this will add up to the variation scale of this parameter~\cite{Dadgour-ICCAD2008}.

Different experimental \cite{TED2016-UCB}, \cite{Matsukawa-2009} and analytical \cite{IEDM2009-Stanford-SRAM}, \cite{Dadgour-ICCAD2008} investigated the impact of process variation elements and compared bulk planar MOSFETs and FinFETs in different technology sizes. While the FinFET devices show less variation due their undoped channels and absence of RDF, the main element of variation will be WFV, which will dramatically increase as the sizes are scaled down as described earlier. In this work we refer to these works and consider the parameters of variation as shown in Fig.~\ref{fig:PV-elements}.

\begin{figure}[]
  \centering
  \subfloat[Redrawn from xXx]{\includegraphics[width=0.4\textwidth]{figures/Dadgour-Fig8.png}\label{fig:f1}}
  \hfill
  \subfloat[Redrawn from yYy]{\includegraphics[width=0.4\textwidth]{figures/Matsukawa-Fig13.png}\label{fig:f2}}
  \caption{(a) Comparison between different sources of random variation for a bulk device. (b) Total random Vth  variation for bulk, FD-SOI and FinFET devices in different technology nodes. The metal material is considered to be TiN for both cases. (c) Linear and saturation Vt variations with their sources for 20-nm-Lg (LSTP) bulk planar MOSFET and FinFET predicted by TCAD considering the smallest AVt for MG FinFET and its increase with scaling LW.} 
  \label{fig:PV-elements}
\end{figure}


% \textbf{How is it handled in CSM:} 
In order to handle process variation, authors in \cite{CSM2} store the CSM lookup tables under the nominal process conditions, and apply polynomial corrections for process variations. The first-order method presented in this paper can provide high accuracy for CMOS devices operating in super-threshold regime. However, for FinFET devices operating in the sub/near-threshold regime, the relationship between the driving current and the gate voltages (and the threshold voltage) becomes exponential. Hence, the polynomial correction method is not sufficient to capture the process variations for FinFET devices operating in the sub/near-threshold regime. To solve this problem, authors in \cite{CSM3} introduce a semi-analytical method which stores the pre-characterized regression coefficients in separate lookup tables.

% \textbf{Why should we consider it? }
% \textbf{How is it handled in STA? }
% \textbf{Why current approaches for handling the process variation are not good?} Just a few lines right now that the reader is fresh about how current methods are not working. 


% Process Variation Resources:
% https://www.design-reuse.com/articles/41330/cmos-soi-finfet-technology-review-paper.html
% GIDL in Doped and Undoped FinFET Devices for Low-Leakage Applications
% Variability Analysis of FinFET-Based Devices and Circuits Considering Electrical Confinement and Width Quantization 
% ITRS 2007 report: https://www.semiconductors.org/resources/2007-international-technology-roadmap-for-semiconductors-itrs/
% ITRS 2007 variation maybe is here: https://www.semiconductors.org/wp-content/uploads/2018/08/2007FEP.pdf
% Tunnel-FET Transistors for 13nm Gate-Length and Beyond
% Investigation and Simulation of Work-Function Variation for III–V Broken-Gap Heterojunction Tunnel FET
% Good article online: http://asic-soc.blogspot.com/2008/03/process-variations-and-static-timing.html

